WINA: Weight Informed Neuron Activation for Accelerating Large Language Model Inference

The growing computational demands of large language models (LLMs) make efficient inference and activation strategies increasingly critical. While recent approaches, such as Mixture-of-Experts (MoE), leverage selective activation but require specialized training, training-free sparse activation methods offer broader applicability and superior resource efficiency through their plug-and-play design. However, many existing methods rely solely on hidden state magnitudes to determine activation, resulting in high approximation errors and suboptimal inference accuracy. To address these limitations, we propose WINA (Weight Informed Neuron Activation), a novel, simple, and training-free sparse activation framework that jointly considers hidden state magnitudes and the column-wise $\ell_2$-norms of weight matrices. We show that this leads to a sparsification strategy that obtains optimal approximation error bounds with theoretical guarantees tighter than existing techniques. Empirically, WINA also outperforms state-of-the-art methods (e.g., TEAL) by up to $2.94\%$ in average performance at the same sparsity levels, across a diverse set of LLM architectures and datasets. These results position WINA as a new performance frontier for training-free sparse activation in LLM inference, advancing training-free sparse activation methods and setting a robust baseline for efficient inference. The source code is available at https://github.com/microsoft/wina.

==> src/fig_acceleraion.tex <==

\begin{figure}[ht!]
    \centering
        \includegraphics[width=0.55\linewidth]{figures/flop_savings_barchart.pdf}
    \caption{\textbf{Computational Savings from WINA.} Percentages indicate the reduction in GFLOPs at the specified sparsity level vs. the full dense model (higher is better). For details, see Table \ref{tbl:gflops}.}
    \label{fig:qwen-overview}
\end{figure}

==> src/tab_acceleration.tex <==

\begin{table}[H]
\centering
\caption{(G)FLOPs over different sparsity across different model architecture.}\label{tab:gflops}
\begin{tabular}{lcccc}
\toprule
Sparsity & Qwen2.5-7B & Llama-2-7B & Llama-3-8B & Phi-4\\
\midrule
Baseline & 7.07 & 6.61 & 7.50 & 14.15  \\
\midrule
0.25 & 5.44 ($\downarrow 23.1\%$) & 4.99 ($\downarrow 24.5\%$) & 5.76 ($\downarrow 23.2\%$) & 10.74($\downarrow 24.1\%$)\\
0.4 &  4.46 ($\downarrow36.9\%$) & 4.02 ($\downarrow39.2\%$) & 4.71 ($\downarrow37.2\%$) & 8.69 ($\downarrow38.6\%$)\\
0.5 & 3.81 ($\downarrow46.1\%$) & 3.37 ($\downarrow49.0\%$) & 4.01 ($\downarrow46.5\%$) & 7.33 ($\downarrow48.2\%$)\\
0.65 & 2.83 ($\downarrow60.0\%$) & 2.40 ($\downarrow63.7\%$) & 2.97 ($\downarrow60.4\%$) & 5.28 ($\downarrow62.7\%$)\\
% \midrule
% {\algacro{} Avg Acc.} & 73.02 & 54.42 & 66.00 & 77.57 \\
\bottomrule
\end{tabular}
\label{tbl:gflops}
\end{table}

==> src/tab_llama2_13b.tex <==
\begin{table*}
  \caption{Results of controlled sparsity experiments over Llama-2-13B}
  \vspace{3pt}
  \label{tab:llama2_13b_sparsity}
  \centering
  % \addtolength{\tabcolsep}{-1pt}
\resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{llccccccc}
    \toprule[0.1em]
    Method & Sparsity & PiQA & Arc-c & WinoGrande & HellaSwag & MMLU & GSM8K & Avg \\
    \midrule
    Baseline & - & - & - & - & - & - & - & - \\ \midrule

\multirow{4}{*}{TEAL~\citep{liu2024trainingfreeactivationsparsitylarge}}  
& 25\% & 84.01 & 48.55 & 72.53 & 79.00 & 51.67 & 22.37 & 59.69 \\
& 40\%  & 79.76 & 48.55 & 71.11 & 77.65 & 49.19 & 19.26 & 57.59 \\
& 50\%  & 78.18 & 47.01 & 69.38 & 75.74 & 45.89 & 15.69 & 55.48 \\
& 65\% & 73.61 & 36.69 & 62.19 & 63.82 & 34.07 & 4.17  & 45.76 \\ 
\midrule

    \multirow{4}{*}{TEAL transform~\citep{liu2024trainingfreeactivationsparsitylarge}}  
& 25\% & 79.92 & 49.40 & 72.77 & 79.38 & 51.47 & 23.81 & 59.46 \\
& 40\% & 79.76 & 49.66 & 71.27 & 79.21 & 50.07 & 22.29 & 58.71 \\
& 50\% & 79.11 & 48.29 & 69.53 & 77.87 & 47.19 & 17.97 & 56.66 \\
& 65\% & 76.82 & 43.52 & 64.09 & 72.19 & 37.13 & 7.43 & 50.22 \\

    \midrule

\multirow{4}{*}{\algacro{}}  
& 25\% & 80.41 & 49.23 & 71.90 & 79.41 & 51.94 & 23.12 & 59.34 \\
& 40\%  & - & - & - & - & - & - & - \\
& 50\%  & - & - & - & - & - & - & - \\
& 65\% & - & - & - & - & - & - & - \\
    \bottomrule[0.1em]
  \end{tabular}
  }
\end{table*}

==> src/tab_model_results.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.25}
\centering
\caption{Perplexity results of controlled sparsity experiments over all models.}
\label{tab:model_results}
\vspace{3pt}
% \addtolength{\tabcolsep}{-1pt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule[0.1em]
\multicolumn{1}{c}{Method (Sparsity)} & \multicolumn{2}{c}{LLaMA-2} & LLaMA-3 & Mistral & Qwen-2.5 & Phi-4\\
\cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
\# Params & {\textbf{7B}} & {\textbf{13B}} & {\textbf{8B}} & {\textbf{7B}} & {\textbf{7B}} & {\textbf{14B}} \\
\midrule
Baseline (0\%) & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX \\ \midrule
TEAL (25\%) & 6.77 & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX    \\
TEAL(transformed) (25\%) & 6.73 & X.XXX & 8.160 & X.XXX & X.XXX & X.XXX    \\
\algacro{} (25\%) &  6.73 & X.XXX & 8.159 & X.XXX & X.XXX & X.XXX  \\ \midrule
TEAL (40\%) & 7.00 & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX   \\
TEAL(transformed) (40\%) & 6.95 & X.XXX & 8.693 & X.XXX & X.XXX & X.XXX    \\
\algacro{} (40\%) & 6.96 & X.XXX & 8.704 & X.XXX & X.XXX & X.XXX  \\ \midrule
TEAL (50\%) & 7.52 & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX   \\
TEAL(transformed) (50\%) & 7.37 & X.XXX & 9.611 & X.XXX & X.XXX & X.XXX    \\
\algacro{} (50\%) & 7.36 & X.XXX & 9.669 & X.XXX & X.XXX & X.XXX   \\ \midrule
TEAL (65\%) & 11.814 & X.XXX & X.XXX & X.XXX & X.XXX & X.XXX \\
TEAL(transformed) (65\%) & X.XXX & X.XXX & 15.706 & X.XXX & X.XXX & X.XXX    \\
\algacro{} (65\%) & 9.580 & X.XXX & 15.832 & X.XXX & X.XXX & X.XXX \\
\bottomrule[0.1em]
\end{tabular}}
\end{table*}

==> src/tab_phi4_14b.tex <==
\begin{table*}
  \caption{Results of controlled sparsity experiments over Phi-4-14B}
  \label{tab:phi4_14b_sparsity}
  \vspace{3pt}
  \centering
  % \addtolength{\tabcolsep}{-1pt}
\resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{llccccccc}
    \toprule[0.1em]
    Method & Sparsity & PiQA & WinoGrande & HellaSwag & Arc-c & MMLU & GSM8K & Avg \\
    \midrule
    Baseline & - & 81.28 & 76.80 & 81.93 & 55.97 & 77.06 & 90.22 & 77.21 \\ \midrule

  \multirow{4}{*}{TEAL~\citep{liu2024trainingfreeactivationsparsitylarge}}  
  & 25\% & 81.07 & 75.45 & 81.92 & 56.23 & 76.63 & 89.84 & 76.86 \\
  & 40\% & 80.79 & 73.80 & 81.21 & 54.95 & 75.10 & 88.02 & 75.98 \\
  & 50\% & 80.63 & 71.98 & 80.06 & 53.84 & 73.52 & 86.13 & 74.36 \\
  & 65\% & 77.64 & 66.06 & 74.26 & 50.77 & 65.17 & 74.37 & 68.71 \\
  \midrule

  \multirow{4}{*}{TEAL-transform} 
  & 25\% & 80.96 & 74.59 & 81.60 & 55.63 & 76.68 & 89.92 & 76.56 \\
  & 40\% & 81.18 & 74.19 & 80.94 & 54.61 & 75.99 & 90.07 & 76.50 \\
  & 50\% & 79.82 & 72.38 & 79.79 & 53.92 & 74.51 & 88.02 & 74.74 \\
  & 65\% & 77.64 & 68.51 & 74.72 & 52.47 & 66.64 & 77.18 & 69.86 \\
  \midrule

\multirow{4}{*}{\textbf{\algacro{} (Ours)}}  
& 25\% & 81.01 & 75.37 & 81.91 & 56.31 & 76.60 & 90.22 & \textbf{77.57} \\
& 40\% & 81.18 & 72.45 & 81.44 & 56.06 & 76.44 & 90.67 & \textbf{76.71} \\
& 50\% & 81.39 & 73.95 & 81.75 & 54.95 & 75.83 & 87.57 & \textbf{75.91} \\
& 65\% & 78.24 & 70.72 & 77.10 & 51.11 & 70.05 & 77.10 & \textbf{70.72} \\
    \bottomrule[0.1em]
  \end{tabular}
  }
\end{table*}



==> src/tab_qwen2.5_7b.tex <==
\begin{table*}[t]
  \caption{Results of controlled sparsity experiments over Qwen-2.5-7B}
  \label{tab:qwen25_7b_sparsity}
  \vspace{3pt}
  \centering
  % \addtolength{\tabcolsep}{-1pt}
    \resizebox{1.0\columnwidth}{!}{
\begin{tabular}{llccccccc}
  \toprule[0.1em]
  Method & Sparsity & PiQA & WinoGrande & HellaSwag & Arc-c & MMLU & GSM8K & Avg \\
  \midrule
  Baseline & - & 79.71 & 72.85 & 78.93 & 51.11 & 71.93 & 83.32 & 72.98 \\ \midrule

  \multirow{4}{*}{TEAL~\citep{liu2024trainingfreeactivationsparsitylarge}}  
  & 25\% & 79.27 & 78.56 & 72.77 & 51.19 & 71.30 & 82.87 & {72.83} \\
  & 40\% & 78.40 & 77.28 & 73.09 & 52.65 & 70.20 & 78.32 & \textbf{71.66} \\
  & 50\% & 78.62 & 75.02 & 69.77 & 51.02 & 67.72 & 71.42 & {68.93} \\
  & 65\% & 73.72 & 63.35 & 62.67 & 42.75 & 54.95 & 34.95 & {55.40} \\ \midrule

  \multirow{4}{*}{TEAL-transform} 
  & 25\% & 80.09 & 72.77 & 78.65 & 51.79 & 71.56 & 83.09 & 72.99 \\
  & 40\% & 79.71 & 72.30 & 77.73 & 51.28 & 69.93 & 77.18 & 71.52 \\
  & 50\% & 78.56 & 68.67 & 75.74 & 50.00 & 67.28 & 71.49 & 68.62 \\
  & 65\% & 76.06 & 61.33 & 67.30 & 44.20 & 56.06 & 32.60 & 56.93 \\ \midrule

  \multirow{4}{*}{\textbf{\algacro{} (Ours)}}  
  & 25\% & 80.05 & 72.69 & 78.58 & 51.37 & 71.51 & 83.93 & \textbf{73.02} \\
  & 40\% & 78.40 & 70.56 & 78.02 & 50.94 & 70.54 & 79.83 & 71.38 \\
  & 50\% & 78.67 & 69.30 & 76.48 & 50.85 & 67.99 & 72.25 & \textbf{69.26} \\
  & 65\% & 76.17 & 61.01 & 70.09 & 42.92 & 59.48 & 38.36 & \textbf{58.34} \\
  \bottomrule[0.1em]
\end{tabular}
  }
\end{table*}

% \begin{table}[t] % [t]表示尽量放在页面顶部
%   \centering
%   \caption{单栏跨栏表格示例}
%   \label{tab:wide}
%   \begin{tabular}{lccr}
%     \toprule
%     Header1 & Header2 & Header3 & Header4 \\
%     \midrule
%     Item1 & 0.25 & 42 & A \\
%     Item2 & 0.67 & 13 & B \\
%     Item3 & 0.92 & 29 & C \\
%     \bottomrule
%   \end{tabular}
% \end{table}

==> tex_arxiv/90_proof.tex <==
\section{Proof}
\jk{Here, we provide the derivation of our theoretical results described in \~}

\subsection{Single-Layer Network}
\paragraph{Model Assumptions.} \jk{Here, we describe the assumption for our theoretical analyses.}
\begin{itemize}[leftmargin=*, itemsep=0pt]
    \item \textbf{Matrix} $W \in \mathbb{R}^{m \times n}$: Elements are independently and identically distributed (i.i.d.) following the standard normal distribution $N(0,1)$.
    \item \textbf{Input vector} $x \in \mathbb{R}^{n}$: Elements are i.i.d. following $N(0,1)$, independent of $W$.
    \item \textbf{Sparsification objective}: Select $k$ elements in $x$ to retain and set the rest to zero, obtaining $x'$, such that $\| Wx' - Wx \|_2$ is minimized.
\end{itemize}

\paragraph{Definitions of Two Sparsification Methods}

\paragraph{TEAL Sparsification}: Define a mask vector $mask_T \in \{0,1\}^n$ for input vector $x$, where:

\[
mask_{T,i} = \begin{cases} 
1, & \text{if } |x_i| < t_{T,p} \\
0, & \text{else}
\end{cases}
\]

where $t_{T,p}$ is the threshold corresponding to the input sparsity level $p$. The sparsified input vector is:

\[
x_T = x \odot mask_T
\]

\textbf{\algacro{} Sparsification}: Define $a \in \mathbb{R}^n$ as the column-wise L2 norm of matrix $W$, where:

\[
a_j = \| W_{:,j} \|_2 = \sqrt{\sum_{i=1}^m W_{i,j}^2}
\]

Define a mask vector $mask_A \in \{0,1\}^n$, where:

\[
mask_{A,i} = \begin{cases} 
1, & \text{if } |x_i \cdot a_i| \text{ in topK elements of } x \odot a \\
0, & \text{else}
\end{cases}
\]

The sparsified input vector is:

\[
x_A = x \odot mask_A
\]

\textbf{Output Error Analysis}

Let $Z_T$ be the set of indices where $mask_T$ is 0, and $Z_A$ be the set where $mask_A$ is 0. The output error for TEAL sparsification is:

\[
\begin{align}\label{equ}
\| W(x_T - x) \|_2^2 &= \left\| \sum_{j \in Z_T} x_j W_{:,j} \right\|_2^2 \\
&= \left( \sum_{j \in Z_T} x_j W_{:,j} \right)^T \left( \sum_{i \in Z_T} x_i W_{:,i} \right) \\
&= \sum_{j \in Z_T} \sum_{i \in Z_T} x_j x_i W_{:,j}^T W_{:,i} \\
&= \sum_{j \in Z_T} x_j^2 \| W_{:,j} \|_2^2 + \sum_{i \neq j \in Z_T} x_j x_i W_{:,j}^T W_{:,i}
\end{align}
\]

The expected output error for TEAL sparsification is:

\[
\begin{align}\label{equ}
e_T &= \mathbb{E}[\| Wx_T - Wx \|_2^2] \\
&= \sum_{j \in Z_T} \mathbb{E}[x_j^2 \| W_{:,j} \|_2^2] + \sum_{i \neq j \in Z_T} \mathbb{E}[x_j x_i W_{:,j}^T W_{:,i}]
\end{align}
\]

Similarly, the expected output error for AdaLoRO sparsification:

\[
\begin{align}\label{equ}
e_A &= \mathbb{E}[\| Wx_A - Wx \|_2^2] \\
&= \sum_{j \in Z_A} \mathbb{E}[x_j^2 \| W_{:,j} \|_2^2] + \sum_{i \neq j \in Z_A} \mathbb{E}[x_j x_i W_{:,j}^T W_{:,i}]
\end{align}
\]

Since $W$ and $x$ are independent with zero-mean elements, the cross-term expectations vanish, and the error expectation is determined solely by the main term:

\[
\begin{align}\label{equ}
e_T &= \sum_{j \in Z_T} \mathbb{E}[x_j^2 \| W_{:,j} \|_2^2] \\
&= \sum_{j \in Z_T} \mathbb{E}[x_j^2 a_j^2]
% \begin{align}\label{equ}
\end{align}
\]

\[
e_A = \sum_{j \in Z_A} \mathbb{E}[x_j^2 \| W_{:,j} \|_2^2] = \sum_{j \in Z_A} \mathbb{E}[x_j^2 a_j^2]
\]


Because AdaLoRO sparsification sets the $k$ smallest $x_j^2 a_j^2$ terms to zero, we have:

\[
\sum_{j \in Z_A} \mathbb{E}[x_j^2 a_j^2] \leq \sum_{j \in Z_T} \mathbb{E}[x_j^2 a_j^2]
\]

Thus, $e_A \leq e_T$, indicating that AdaLoRO sparsification achieves lower expected error than TEAL sparsification, and it is superior to any other sparsification method.

\subsection{Two-Layer Network}

\textbf{Model Assumptions}

\begin{itemize}
    \item \textbf{Matrix} $W^{(1)} \in \mathbb{R}^{m \times n}$: Elements are i.i.d. following $N(0,1)$.
    \item \textbf{Matrix} $W^{(2)} \in \mathbb{R}^{h \times m}$: Elements are i.i.d. following $N(0,1)$, independent of $W^{(1)}$.
    \item \textbf{Input vector} $x \in \mathbb{R}^n$: Elements are i.i.d. following $N(0,1)$, independent of $W^{(1)}$ and $W^{(2)}$.
    \item \textbf{Sparsification objective}: Apply sparsification masks $mask^{(1)}$ and $mask^{(2)}$ to the inputs of $W^{(1)}$ and $W^{(2)}$, retaining $k$ elements, to minimize the expected output error:
    \[
    \mathbb{E}[\| W^{(2)}(W^{(1)}(x \odot mask^{(1)}) \odot mask^{(2)}) - W^{(2)} W^{(1)} x \|_2]
    \]
\end{itemize}

\textbf{Definitions of Two Sparsification Methods}

\textbf{TEAL Sparsification}: Define the input mask vector $mask_T^{(1)} \in \{0,1\}^n$ of $W^{(1)}$ for input vector $x$, where:

\[
mask_{T,i}^{(1)} = \begin{cases} 
1, & \text{if } |x_i| \text{ in topK elements} \\
0, & \text{else}
\end{cases}
\]

The sparsified input vector is:

\[
x_T^{(1)} = x \odot mask_T^{(1)}
\]

The output vector of $W^{(1)}$ is:

\[
y_T^{(1)} = W^{(1)} x_T^{(1)}
\]

Define the input mask vector $mask_T^{(2)} \in \{0,1\}^m$ for $W^{(2)}$, where:

\[
mask_{T,i}^{(2)} = \begin{cases} 
1, & \text{if } |y_T^{(1)}| \text{ in topK elements} \\
0, & \text{else}
\end{cases}
\]

The sparsified input vector for $W^{(2)}$ is:

\[
x_T^{(2)} = y_T^{(1)} \odot mask_T^{(2)}
\]

\textbf{AdaLoRO Sparsification}: Define $a^{(1)} \in \mathbb{R}^n$ as the column-wise L2 norm of $W^{(1)}$, and $a^{(2)} \in \mathbb{R}^m$ as the column-wise L2 norm of $W^{(2)}$, where:

\[
a_j^{(1)} = \| W_{:,j}^{(1)} \|_2 = \sqrt{\sum_{i=1}^m W_{i,j}^{(1)2}}
\]
\[
a_j^{(2)} = \| W_{:,j}^{(2)} \|_2 = \sqrt{\sum_{i=1}^m W_{i,j}^{(2)2}}
\]

Define the input mask vector $mask_A^{(1)} \in \{0,1\}^n$ for $W^{(1)}$, where:

\[
mask_{A,i}^{(1)} = \begin{cases} 
1, & \text{if } |x_i \odot a_i^{(1)}| \text{ in topK elements of } x \odot a \\
0, & \text{else}
\end{cases}
\]

The sparsified input vector for $W^{(1)}$ is:

\[
x_A^{(1)} = x \odot mask_A^{(1)}
\]

The output vector of $W^{(1)}$ is:

\[
y_A^{(1)} = W^{(1)} x_A^{(1)}
\]

Define the input mask vector $mask_A^{(2)} \in \{0,1\}^m$ for $W^{(2)}$, where:

\[
mask_{A,i}^{(2)} = \begin{cases} 
1, & \text{if } |y_A^{(1)} \odot a_i^{(2)}| \text{ in topK elements} \\
0, & \text{else}
\end{cases}
\]

The sparsified input vector for $W^{(2)}$ is:

\[
x_A^{(2)} = y_A^{(1)} \odot mask_A^{(2)}
\]

\textbf{Output Error Analysis}

Let $Z_T$ be the set of indices where $mask_T$ is 0, and $Z_A$ be the set where $mask_A$ is 0.

The output error for TEAL sparsification is:

\[
\begin{align}\label{equ}
\| &y_T^{(2)} - y \|_2 \\
= \| &W^{(2)} W^{(1)} (x \odot mask_T^{(1)}) \odot mask_T^{(2)} - W^{(2)} W^{(1)} x \|_2 \\
= \| &W^{(2)} [W^{(1)} (x \odot mask_T^{(1)}) - W^{(1)} x \\
&+ W^{(1)} (x \odot mask_T^{(1)}) \odot (mask_T^{(2)} - 1)] \|_2 \\
= \| &W^{(2)} (\underbrace{W^{(1)} x_T^{(1)} - W^{(1)} x}_{error_T^{(1)}} + \underbrace{y_T^{(1)} \odot mask_T^{(2)} - y_T^{(1)}}_{error_T^{(2)}}) \|_2
\end{align}
\]

Where $error_T^{(1)} = W^{(1)} x_T^{(1)} - W^{(1)} x$ represents the first-layer error, and $error_T^{(2)} = y_T^{(1)} \odot mask_T^{(2)} - y_T^{(1)}$ represents the second-layer error.

The expected output error is:

\[
\begin{align}\label{equ}
e_T = &\mathbb{E}[\| W^{(2)} (error_T^{(1)} + error_T^{(2)}) \|_2^2] \\
&= \mathbb{E}[\| W^{(2)} error_T^{(1)} \|_2^2] + \mathbb{E}[| W^{(2)} error_T^{(2)} \|_2^2] \\
&+ 2 \mathbb{E}[\| error_T^{(1)T} W^{(2)T} W^{(2)} error_T^{(2)} \|_2^2]
\end{align}
\]

Since all variables are i.i.d., the cross-term expectation is zero. Thus:

\[
\begin{align}\label{equ}
e_T &= \mathbb{E}[\| W^{(2)} error_T^{(1)} \|_2^2] + \mathbb{E}[\| W^{(2)} error_T^{(2)} \|_2^2] \\
&= \| W^{(2)} \|_2^2 \cdot \mathbb{E}[\| error_T^{(1)} \|_2^2] + \mathbb{E}[\| W^{(2)} error_T^{(2)} \|_2^2]
\end{align}
\]

Similarly, the expected error for AdaLoRO sparsification is:

\[
e_A = \| W^{(2)} \|_2^2 \cdot \mathbb{E}[\| error_A^{(1)} \|_2^2] + \mathbb{E}[\| W^{(2)} error_A^{(2)} \|_2^2]
\]

Here, $\mathbb{E}[\| error_T^{(1)} \|_2^2]$ and $\mathbb{E}[\| error_A^{(1)} \|_2^2]$ correspond to the expected errors in Situation 1. Therefore:

\[
\mathbb{E}[\| error_A^{(1)} \|_2^2] \leq \mathbb{E}[\| error_T^{(1)} \|_2^2]
\]

Next, we compare $\mathbb{E}[\| error_T^{(2)} \|_2^2]$ and $\mathbb{E}[\| error_A^{(2)} \|_2^2]$. Let $Z_T$ be the set of indices where $mask_T^{(2)}$ is 0, and $Z_A$ be the set of indices where $mask_A^{(2)}$ is 0.

For TEAL sparsification:

\[
\begin{align}\label{equ}
&\mathbb{E}[\| W^{(2)} error_T' \|_2^2] \\
= &\mathbb{E}[\| W^{(2)} (y_T^{(1)} \odot mask_T^{(2)}) - W^{(2)} y_T^{(1)} \|_2^2] \\
= &\mathbb{E}[\sum_{j \in Z_T} y_{T,j}^{(1)2} \cdot \| W_{:,j}^{(2)} \|_2^2] = \mathbb{E}[\sum_{j \in Z_T} y_{T,j}^{(1)2} \cdot a_j^{(2)2}]
\end{align}
\]

For AdaLoRO sparsification:

\[
\mathbb{E}[\| W^{(2)} error_A' \|_2^2] = \mathbb{E}[\sum_{j \in Z_A} y_{A,j}^{(1)2} \cdot a_j^{(2)2}]
\]

From Situation 1, we know that for the same intermediate output $y_{A,j}^{(1)}$, using $mask_A^{(2)}$ results in smaller expected error than using $mask_T^{(2)}$, i.e.:

\[
\mathbb{E}[\sum_{j \in Z_A} y_{A,j}^{(1)2} \cdot a_j^{(2)2}] \leq \mathbb{E}[\sum_{j \in Z_T} y_{A,j}^{(1)2} \cdot a_j^{(2)2}]
\]

Thus, if the following inequality holds:

\[
\mathbb{E}[\sum_{j \in Z_T} y_{A,j}^{(1)2} \cdot a_j^{(2)2}] \leq \mathbb{E}[\sum_{j \in Z_T} y_{T,j}^{(1)2} \cdot a_j^{(2)2}]
\]

then we have:

\[
e_A = \mathbb{E}[\sum_{j \in Z_A} y_{A,j}^{(1)2} \cdot a_j^{(2)2}] \leq \mathbb{E}[\sum_{j \in Z_T} y_{T,j}^{(1)2} \cdot a_j^{(2)2}] = e_T
\]

We now prove this inequality:

\[
\begin{align}\label{equ}
&\mathbb{E}[\sum_{j \in Z_T} y_{A,j}^{(1)2} \cdot a_j^{(2)2}] \\
= &\sum_{j \in Z_T} \mathbb{E}[y_{A,j}^{(1)2}] \cdot a_j^{(2)2} \\
= &\sum_{j \in Z_T} \mathbb{E}[(W_{j,:}^{(1)} x \odot mask_A^{(1)})^2] \cdot a_j^{(2)2}
\end{align}
\]

Here, $W_{j,:}^{(1)}$ can be viewed as a $1 \times m$ matrix, and $W_{j,:}^{(1)} x \odot mask_T^{(1)}$, $W_{j,:}^{(1)} x \odot mask_A^{(1)}$ correspond to the case where $n=1$ in Situation 1. Therefore:

\[
\mathbb{E}[(W_{j,:}^{(1)} (x \odot mask_A^{(1)}))^2] \leq \mathbb{E}[(W_{j,:}^{(1)} (x \odot mask_T^{(1)}))^2]
\]

Thus:

\[
\sum_{j \in Z_T} \mathbb{E}[(W_{j,:}^{(1)} x \odot mask_A^{(1)})^2] \cdot a_j^{(2)2} \leq \sum_{j \in Z_T} \mathbb{E}[(W_{j,:}^{(1)} x \odot mask_T^{(1)})^2] \cdot a_j^{(2)2}
\]

Consequently:

\[
e_A = \mathbb{E}[\sum_{j \in Z_A} y_{A,j}^{(1)2} \cdot a_j^{(2)2}] \leq \mathbb{E}[\sum_{j \in Z_T} y_{T,j}^{(1)2} \cdot a_j^{(2)2}] = e_T
\]

==> tex_arxiv/proof_theorem_3.2_old.tex <==
\subsection{Proof of Theorem 3.2}\label{app:thm3.2}

\paragraph{Proof.} We prove this by mathematical induction. 
\paragraph{Step 1: Base case $N=2$.} The output error for sparse activation parameterized via mask $\bm{g}$ is:
\begin{align*}\label{equ}
&\norm{\bm{y}_{\bm{g}}^{(2)} - \bm{y}^{(2)}} \\
= &\norm{W^{(2)} (\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)}) - W^{(2)} \bm{y}^{(1)}} \\
= &\norm{W^{(2)} (\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)}) - W^{(2)}\bm{y}_{\bm{g}}^{(1)} + W^{(2)}\bm{y}_{\bm{g}}^{(1)}-W^{(2)} \bm{y}^{(1)}} \\
= &\norm{W^{(2)}{(\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}}^{(1)})} + W^{(2)}{(\bm{y}_{\bm{g}}^{(1)} - \bm{y}^{(1)})}}\\
= &\norm{W^{(2)}{(\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}}^{(1)}}) + W^{(2)}(W^{(1)} \bm{x}\odot \bm{g}^{(1)} - W^{(1)} \bm{x})}
\end{align*}
Let: 
$$
\Delta^{(1)} = \text{diag}(\bm{g}^{(1)} - 1),\quad \Delta^{(2)} = \text{diag}(\bm{g}^{(2)} - 1), \quad M^{(1)} = \text{diag}(\bm{g}^{(1)}).
$$
Then, let $\bm{v}$ and $\bm{u}$ be 
\begin{align*}
\bm{v} &=W^{(2)}(\bm{y}_{\bm{g}}^{(1)}\odot(\bm{g}^{(2)}-{1}))\\
&=W^{(2)}(W^{(1)}(\bm{x}\odot \bm{g}^{(1)})\odot(\bm{g}^{(2)}-1)) \\
&=W^{(2)}\Delta^{(2)}W^{(1)}M^{(1)}\bm{x}\\
\bm{u} &=W^{(2)}W^{(1)}(\bm{x}\odot(\bm{g}^{(1)}-1))\\
&=W^{(2)}W^{(1)}\Delta^{(1)}\bm{x}. \\
\end{align*}
Since $\E{\norm{\bm{u} + \bm{v}}^2} = \E{\norm{\bm{u}}^2} + \E{\norm{\bm{v}}^2} + 2\E{(\bm{u}^\top\bm{v})}$, the expected value of the cross-term is:
\begin{align*}
\E[\bm{u}^\top\bm{v}] &= \E[\bm{x}^\top\Delta^{(1)}(W^{(1)})^\top(W^{(2)})^\top(W^{(2)})\Delta^{(2)}W^{(1)}M^{(1)}\bm{x}] \\
&= \E[\text{tr}(W^{(2)}\Delta^{(2)}W^{(1)}M^{(1)}\bm{x}\bm{x}^\top\Delta^{(1)}(W^{(1)})^\top(W^{(2)})^\top)] \\
&= \text{tr}\left(W^{(2)}\E[\Delta^{(2)}]W^{(1)}\E[M^{(1)}\Delta^{(1)}]\E[\bm{x}\bm{x}^\top](W^{(1)})^\top(W^{(2)})^\top\right)
\end{align*} 
Since $\E[M_1\Delta_1]=\E[\bm{g}^{(1)}\odot(\bm{g}^{(1)}-1)]=0$, the cross-term expectation $\E[\bm{u}^\top\bm{v}]$ is zero. Thus, the expected output deviation via sparse activation $\bm{g}$,
\begin{equation}
\begin{split}
e^{(2)}&=\E[\norm{\bm{u}+\bm{v}}^2]\\    
&=\E[\norm{W^{(2)}{(\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}}^{(1)}})}^2] +\E[\norm{W^{(2)}(W^{(1)} \bm{x}\odot \bm{g}^{(1)} - W^{(1)} \bm{x})}^2]
\end{split}
\end{equation}
Upon Lemma~\ref{lemma.single_layer}, we have that
$$
\mathbb{E}[\| W^{(2)}(W^{(1)} \bm{x}\odot \bm{g}_{\text{\algacro{}}}^{(1)} - W^{(1)} \bm{x}) \|^2] \leq \mathbb{E}[\| W^{(2)}(W^{(1)} \bm{x}\odot \bm{g}_{\text{TEAL}}^{(1)} - W^{(1)} \bm{x}) \|^2]
$$
Next, we compare $\mathbb{E}[\|W^{(2)}(\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}}^{(1)})\|^2]$ given $\bm{g}_\text{\algacro{}}^{(2)}$ and $\bm{g}_\text{TEAL}^{(2)}$.
\begin{align*}
&\ \mathbb{E}[\|W^{(2)}(\bm{y}_{\bm{g}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}}^{(1)})\|^2]\\
=&\ \E[{\sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(2)})}\sum_{i\in \mathcal{I}^{=0}(\bm{g}^{(2)})} \bm{y}_j^{(1)}\bm{y}_i^{(1)}\,(W_{:,j}^{(2)})^\top W_{:,i}^{(2)}}]\\
= &\E[{\sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(2)})} (\bm{y}_j^{(1)})^2\|W_{:,j}^{(2)}\|^2 + \sum_{\substack{i,j\in \mathcal{I}^{=0}(\bm{g}^{(2)})\\i\neq j}} \bm{y}_j^{(1)}\bm{y}_i^{(1)}\,(W_{:,j}^{(2)})^T W_{:,i}^{(2)}}]\\
= &\ \sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(2)})}{(\bm{c}_j^{(2)})^2\E{(\bm{y}_{j}^{(1)})^2}} + \sum_{\substack{i,j\in \mathcal{I}^{=0}(\bm{g}^{(2)})\\i\neq j}}({W_{:,j}^{(2)})^\top W_{:,i}^{(2)}\E[{\bm{y}_j^{(1)}\bm{y}_i^{(1)}}]}\\
= &\ \sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(2)})}{(\bm{c}_j^{(2)})^2\E{(\bm{y}_{j}^{(1)})^2}},
\end{align*}
where the last line is due to $W^{(2)}$ is column-orthogonal, the cross-term's expectation is zero.

Because \algacro{} sparsification sets the $k$ smallest $(\bm{y}_j^{(1)}c_j^{(2)})^2$ terms to zero, we have:
$$
\mathbb{E}[\|W^{(2)}(\bm{y}_{\bm{g}_\text{\algacro{}}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}_\text{\algacro{}}}^{(1)})\|^2]\leq \mathbb{E}[\|W^{(2)}(\bm{y}_{\bm{g}_\text{TEAL}}^{(1)} \odot \bm{g}^{(2)} - \bm{y}_{\bm{g}_{\text{TEAL}}}^{(1)})\|^2]
$$
Therefore, we have that 
$$
e_{\text{\algacro{}}}^{(2)}\leq e_{\text{TEAL}}^{(2)}.
$$
\paragraph{Step 2: Inductive proof for $N>2$.}
Assume for some $N\ge2$ that
$$
e_{\text{\algacro{}}}^{(N)}\leq e_{\text{TEAL}}^{(N)}.
$$
Define the exact output of $(N+1)$ layer network:
$$
\bm{y} = W^{(N+1)} \bm{y}^{(N)}, \quad \bm{y}^{(N)} = W^{(N)}\cdots W^{(1)}\bm{x}
$$
The output via mask $\bm{g}^{(N+1)}$ is that
\begin{align*}
&\ \bm{y}_{\bm{g}}^{(N+1)} - \bm{y} \\
=\ &\ W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}^{(N+1)}) - W^{(N+1)}\bm{y}^{(N)} \\
=\ &\ W^{(N+1)}((\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}^{(N+1)} ) - \bm{y}_{\bm{g}}^{(N)}) + W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} - \bm{y}^{(N)})
\end{align*}
The expected output deviation is:
\begin{equation}
e_{\bm{g}}^{N+1}=\E\|W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}^{(N+1)} - \bm{y}_{\bm{g}}^{(N)})\|^2 + \E\|W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} - \bm{y}^{(N)})\|^2,
\end{equation}
the cross-term zeros out because of the assumption. 

Upon induction assumption, for the second term, we have that 
\begin{equation}
\E\|W^{(N+1)}(\bm{y}_{\bm{g}_\text{\algacro{}}}^{(N)} - \bm{y}^{(N)})\|^2\leq \E\|W^{(N+1)}(\bm{y}_{\bm{g}_\text{TEAL}}^{(N)} - \bm{y}^{(N)})\|^2.
\end{equation}
For the first term, we have that 
\begin{align*}
&\ \mathbb{E}[\|W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}^{(N+1)} - \bm{y}_{\bm{g}}^{(N)})\|^2]\\
=&\ \E[{\sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(N+1)})}\sum_{i\in \mathcal{I}^{=0}(\bm{g}^{(N+1)})} \bm{y}_j^{(N)}\bm{y}_i^{(N)}\,(W_{:,j}^{(N+1)})^\top W_{:,i}^{(N+1)}}]\\
= &\ \sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(N+1)})}{(\bm{c}_j^{(N+1)})^2\E{(\bm{y}_{j}^{(N)})^2}} + \sum_{\substack{i,j\in \mathcal{I}^{=0}(\bm{g}^{(N+1)})\\i\neq j}}({W_{:,j}^{(N+1)})^\top W_{:,i}^{(N+1)}\E[{\bm{y}_j^{(N)}\bm{y}_i^{(N)}}]}\\
= &\ \sum_{j\in \mathcal{I}^{=0}(\bm{g}^{(N+1)})}{(\bm{c}_j^{(N+1)})^2\E{(\bm{y}_{j}^{(N)})^2}},
\end{align*}
where the last line is due to $W^{(N+1)}$ is column-orthogonal, the cross-term's expectation is zero.

Since \algacro{} retains the $k$ largest $|\bm{y}_j^{(N)}\bm{c}_j^{N+1}|$, thus:
\begin{equation}
\mathbb{E}[\|W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}_\text{\algacro{}}^{(N+1)} - \bm{y}_{\bm{g}}^{(N)})\|^2]\leq \mathbb{E}[\|W^{(N+1)}(\bm{y}_{\bm{g}}^{(N)} \odot \bm{g}_\text{TEAL}^{(N+1)} - \bm{y}_{\bm{g}}^{(N)})\|^2].
\end{equation}
Consequently, we reach the conclusion that
\begin{align}
e_\text{\algacro{}}^{(N+1)}\leq e_\text{TEAL}^{(N+1)}.
\end{align}



